Non-preemptive Scheduling in a Smart Grid Model and its Implications on Machine Minimization

We study a scheduling problem arising in demand response management in smart grid. Consumers send in power requests with a flexible feasible time interval during which their requests can be served. The grid controller, upon receiving power requests, schedules each request within the specified interval. The electricity cost is measured by a convex function of the load in each timeslot. The objective is to schedule all requests with the minimum total electricity cost. Previous work has studied cases where jobs have unit power requirement and unit duration. We extend the study to arbitrary power requirement and duration, which has been shown to be NP-hard. We give the first online algorithm for the general problem, and prove that the problem is fixed parameter tractable. We also show that the online algorithm is asymptotically optimal when the objective is to minimize the peak load. In addition, we observe that the classical non-preemptive machine minimization problem is a special case of the smart grid problem with min-peak objective, and show that we can solve the non-preemptive machine minimization problem asymptotically optimally.

==> peak_long.tex <==
\renewcommand{\Alg}{{\mathcal{G}}}

\section{Minimizing peak and non-preemptive machine minimization}
\label{sec:peak}

In this section, we we extend our algorithms to solve other problems. %, the smart grid scheduling problem with objective to minimize the peak power demand and the machine minimization problem.
We \hhl{show} that the online algorithm introduced in Section~\ref{sec:general} performs well on the problems which objective is to minimize the peak power demand or number of machines used. 
We also find that the exact algorithm introduced in Section~\ref{sec:exact} can solve other demand response management problems with different objective functions, and hence we can prove these problems are all fixed-parameter tractable with respect to the same group of parameters. 

\runtitle{The $\peak$ problem.} 
The input of the $\peak$ problem is a set of jobs where each job has a power request $\h$, time duration $\w$, release time $\Rtime{}$, and deadline $\Dline{}$. A job should be finished between its feasible interval $[\Rtime{}, \Dline{})$.
The goal is to feasibly serve all jobs without preemption such that the maximum \hhl{load} over time horizon is minimized. 

The $\peak$ problem has been proven to be NP-hard by Tang et al.~\cite{tang2013smoothing}. 
Yaw et al.~\cite{DBLP:conf/smartgridcomm/YawMML14} proposed a $4$-approximation algorithm for input jobs with common feasible interval and an $O(\log \frac{\wmax}{\wmin})$-approximation algorithm for jobs with agreeable deadlines.

\hhl{
We now introduce another optimization problem, the non-preemption \emph{machine minimization} problem. 
}

\hhl{
\runtitle{The $\minimization$ problem.} 
The input of the $\minimization$ problem is a set of jobs where each job has processing time $\Work{}$, release time $\Rtime{}$, and deadline $\Dline{}$. 
Each job has to be scheduled on one of the infinite number of machines without preemption. 
For each machine, at any time there should be at most one job executed on it. 
%There are infinite number of machines, an each job has to be scheduled on a machine such that in its execution interval (which is inside the interval between its release time and deadline) there is no other jobs assigned on the same machine. 
The goal is to minimize the number of opened machines. 
%The non-preemptive machine minimization problem is a special case of the smart grid scheduling problem with objective of minimizing the peak. 
}

\hhl{
The $\minimization$ problem can be seen as a special case of the $\peak$ problem with special input set where jobs have unit height. 
Saha~\cite{DBLP:conf/fsttcs/Saha13} proved that any online algorithm for the non-preemptive Machine Minimization problem has competitive ratio at least $\log_3 \frac{\wmax}{{\wmin}}$. 
Since the Machine Minimization problem is a special case of the $\peak$ problem where jobs have unit height, the lower bound also holds for the $\peak$ problem. 
}

\hhl{
Saha also proposed an $O(\log \frac{p_{\max}}{p_{\min}})$-competitive online algorithm in~\cite{DBLP:conf/fsttcs/Saha13}. 
The algorithm basically classified jobs by their processing times and applies the constant approximation non-preemptive machine minimization algorithm \fhl{proposed by Chuzhoy and Codenotti~\cite{DBLP:conf/approx/ChuzhoyC09}} for each class. Unfortunately, the authors~\cite{DBLP:conf/approx/ChuzhoyC09a} have retreated the results as they have identified a mistake in the analysis which invalidates the claimed approximation ratio and as a result the best approximation ratio for the problem remains $O(\sqrt{\frac{\log n}{\log\log n}})$.
%that there are something wrong in their analysis of the algorithm~\cite{DBLP:conf/approx/ChuzhoyC09a}, therefore best current approximation ratio for this problem remains $O(\sqrt{\frac{\log n}{\log\log n}})$}. 
Hence it remains unknown if there existed an asymptotically optimal algorithm for the non-preemptive machine minimization problem. 
We prove that the online algorithm $\Alg$ proposed in Section~\ref{sec:general} is asymptotically optimal for the $\peak$ problem. 
}

In this section, we consider the $\peak$ problem in the online model. 
%Saha~\cite{DBLP:conf/fsttcs/Saha13}\footnote{Saha also proposed an $O(\log \frac{p_{\max}}{p_{\min}})$-competitive online algorithm in~\cite{DBLP:conf/fsttcs/Saha13}. 
%The algorithm basically classified jobs by their processing times and applies the constant approximation non-preemptive machine minimization algorithm proposed by Chuzhoy and Codenotti~\cite{DBLP:conf/approx/2009} for each class. Unfortunately, the authors~\cite{DBLP:conf/approx/ChuzhoyC09a} have retreated the results as they have identified a mistake in the analysis which invalidates the claimed approximation ratio and as a result the best approximation ratio for the problem remains $O(\sqrt{\frac{\log n}{\log\log n}})$.
%%that there are something wrong in their analysis of the algorithm~\cite{DBLP:conf/approx/ChuzhoyC09a}, therefore best current approximation ratio for this problem remains $O(\sqrt{\frac{\log n}{\log\log n}})$}. 
%Hence it remains unknown if there existed an asymptotically optimal algorithm for the non-preemptive machine minimization problem. 
%} 
%proved that any online algorithm for the non-preemptive Machine Minimization problem has competitive ratio at least $\log_3 \frac{\wmax}{{\wmin}}$. 
%Since the Machine Minimization problem is a special case of the $\peak$ problem where jobs have unit height, the lower bound also holds for the $\peak$ problem. 
%We prove that the online algorithm $\Alg$ proposed in Section~\ref{sec:general} is asymptotically optimal for the $\peak$ problem. 
More specifically, we use the online strategy to solve the $\peak$ problem by using the adapted $\BKP$ algorithm, $\newBKP$ (see Section~\ref{sec:vertical}), as the reference algorithm. 
\hhl{Bansal et al.~\cite{DBLP:journals/jacm/BansalKP07} proved that the $\BKP$ algorithm is $e$-competitive with respect to maximum speed.}

%Bansal et al.~\cite{DBLP:journals/jacm/BansalKP07} proved the following lemma:
%
%\begin{lemma}[\textbf{\cite{DBLP:journals/jacm/BansalKP07}}]
%\label{lm:BKP_peak}
%The $\BKP$ algorithm is $e$-competitive with respect to maximum speed.
%\end{lemma}

According to Lemma~\ref{lm:bkp_load}, we have the following lemma:
\begin{observation}
\label{lem:BKPL_peak}
The $\newBKP$ algorithm is $e(1+e)$-competitive with respect to maximum speed.
\end{observation}

\begin{proof}
By Lemma~\ref{lm:bkp_load}, for any integral $t$ and $0<\Delta<1$, $\load(\BKP, t+\Delta) \leq (1+e)\cdot \load(\BKP,t)$. 
Also, by $\newBKP$, $\load(\newBKP,t) \geq \load(\BKP,t+\Delta)$ for any $0<\Delta<1$. 
Hence, \hhl{$\p(\newBKP) \leq (1+e)\cdot \p(\BKP)$}.
\end{proof}

Also, the $\YDS$ algorithm guarantees that maximum speed is minimized~\cite{DBLP:journals/jacm/BansalKP07}. 
Let function $\p(\Sch)$ denote the maximum \hhl{load} of schedule $\Sch$. 
More formally, $\p(\Sch) = \max_{t} \Load{\Sch}{t}$. 
Similar to Observation~\ref{thm:opt_dvs_grid}, $\YDS$ gives a lower bound for the $\peak$ problem. 

\begin{observation}
\label{ob:opt_peak}
Let $\Opt_D$ and $\Opt_G$ be the optimal schedule for the $\dvs$ and $\peak$ problem, respectively. 
Given a job set $\Jobsetij{G}$ for the $\peak$ problem. \hhl{Let $\Jobsetij{O}$ denote the job set after converting $\Jobsetij{G}$ into a job set for the $\dvs$ problem (see Section~\ref{sec:prelim})}, $\p(\Opt_D(\Jobsetij{D})) \leq \p(\Opt_G(\Jobsetij{G}))$. 
\end{observation}

%\runtitle{Revisit the online algorithm $\Alg$ for general input.} 
%Recall that in Section~\ref{Sec:online_general}, we solve the general case by generalizing the online algorithm for special input. 
%We repeat the algorithm $\Alg$ and the Procedures and Transformations in this section. 
%The algorithm $\AlgV$ can schedule unit-width jobs with promising performance by referencing to an arbitrary feasible online algorithm for the $\dvs$ problem. 
%To solve the $\peak$ problem, we reference the $\BKP$ algorithm. 
%By generalizing $\AlgV$, we have online algorithm~$\AlgUV$ for jobs with uniform width. By further generalizing~$\AlgUV$, we have online algorithm~$\Alg$ for jobs with arbitrary widths and arbitrary heights. 
%
%We denote $\niceJobsetij{}$ as set of \emph{nice} jobs, that is, the set of jobs with uniform width. 
%Also, we denote $\alignJobsetij{}$ as the set of nice jobs with their release times and deadlines at $i\cdot \w$ for some integers $i$ where $\w$ is the width of jobs. 
%A job set $\Jobset$ can be transformed into a corresponding nice job set $\niceJobsetij{}$ by Procedure $\convert$; a nice job set $\niceJobsetij{}$ where jobs have long enough feasible intervals can be transformed into a corresponding $\alignJobsetij{}$ by Procedure $\convertfi$:
%
%\runtitle{Procedure $\convertw$.}
%Given a job set $\Jobset$ where jobs have arbitrary widths and arbitrary heights, we define the procedure $\convertw$ to transform each job $\Job{}\in \Jobset$ into a \emph{nice} job $\niceJob{}$ as follows. 
%We denote the resulting nice job set by $\niceJobsetij{}$. 
%Suppose $\Job{}$ has width $2^{p-1}<\Width{}\leq 2^p$ for an integer $p> 1$. 
%We modify its width, release time and deadline.
%\begin{itemize}
%\item $\niceWidth{} \leftarrow 2^p$;
%\item $\niceRtime{} \leftarrow \Rtime{}$;
%\item $\niceDline{} \leftarrow \niceRtime{} + \max\{\Dline{}-\Rtime{}, 2^p\}$.
%\end{itemize}
%
%\runtitle{Procedure $\convertfi$.} 
%Given a loose job set $\niceJSloose$ where jobs have uniform width $\w$ and $|\Interval{}|>2\cdot \w$ for all $\Job{}\in \niceJSloose$. 
%We define the procedure $\convertfi$ to transform each loose job $\Job{} \in \niceJSloose$ into a job $\uwaJ{}$ with release time and deadline ``aligned'' as follows. We denote the resulting job set by $\alignJobsetij{}$. 
%\begin{itemize}
%\item $\alignRtime{} \leftarrow \min_{i\geq 0} \{i\cdot \w \mid i\cdot \w \geq\Rtime{}\}$;
%\item $\alignDline{} \leftarrow \max_{i\geq 0} \{i\cdot \w \mid i\cdot \w \leq\Dline{}\}$.
%\end{itemize}
%
%The algorithm $\Alg$ runs like the following. 
%For the input job set $\Jobset$ where jobs with arbitrary widths and arbitrary heights, the jobs are classified by their widths and each class of jobs are scheduled independently. 
%In each class, the jobs' widths are rounded up to a certain constant by $\convert$ and form a new set $\niceJobsetij{p}$ where the jobs have uniform width $2^p$. 
%Then the algorithm $\AlgUV$ for uniform-width jobs is performed on each subset $\niceJobsetij{p}$ ob jobs. 
%In $\AlgUV$, jobs (with uniform width) are classified by the length of their feasible intervals. 
%A job is \emph{loose} if the length of its feasible interval is at least twice as its width; other wise, the job is \emph{tight}. 
%The tight jobs are executed once they arrived. 
%On the other hand, the loose jobs' release times and deadlines are aligned by $\convertfi$ such that although some of the time which is feasible for the jobs are sacrificed, the jobs can be treated as unit-width input. 
%The jobs after $\convertfi$ form a set $\alignJobsetij{p}$. 
%Then the algorithm $\AlgV$ can be employed on $\alignJobsetij{}$. 
%By Transformation $\freeS$, the schedule for unit-width jobs generated by $\AlgV$ can be transformed into a schedule for uniform-width jobs. And by Transformation $\shrinkS$, the schedule generated by $\AlgUV$ can be transformed into a schedule for general input, that is, the original input set $\Jobsetij{}$. 
%
%For the analysis, we show that the Transformations $\freeS$ and $\shrinkS$ do not increase the cost of the resulting schedule. 
%On the other hand, by the Transformation $\alignS$ and Transformation $\relaxS$ we prove that the rounding up of widths of the jobs and aligning the feasible intervals of the jobs (which sacrifices parts of feasible intervals) do not increase the competitive ratio dramatically. 
%
%\medskip
%
%For completeness, we list the mentioned transformations below. 
%For a schedule $\Schij{}$ for a job set $\Jobsetij{}$, we denote $\niceSchij{}$ as a schedule for the corresponding $\niceJobsetij{}$ generated by $\convert$; we also denote $\alignSchij{}$ as a schedule for the corresponding $\alignJobsetij{}$ generated by $\convertfi$. 
%
%\runtitle{Transformation $\freeS$.}
%$\freeS$ transforms a schedule $\alignSchij{}$ for jobs with uniform width and aligned feasible intervals into a schedule $\niceSchij{}$ for the corresponding nice job set.
%\begin{itemize}
%\item $\Stime{\niceSchij{}}{\Job{}} \leftarrow \Stime{\alignSchij{}}{\alignJob{}}$;
%\item $\Etime{\niceSchij{}}{\Job{}} \leftarrow \Etime{\alignSchij{}}{\alignJob{}}$.
%\end{itemize}
%
%\runtitle{Transformation $\shrinkS$.}
%$\shrinkS$ converts a schedule $\niceSchij{}$ for a nice job set $\niceJobsetij{}$ to a schedule $\Sch$ for the corresponding job set $\Jobset$.
%We set
%\begin{itemize}
%\item $\Stime{\Schij{}}{\Job{}} \leftarrow \Stime{\niceSchij{}}{\niceJob{}}$;
%\item $\Etime{\Schij{}}{\Job{}} \leftarrow \Stime{\Schij{}}{\Job{}} + \Width{} $, 
%therefore, $\Etime{\Schij{}}{\Job{}} \leq \Etime{\niceSchij{}}{\niceJob{}}$.
%\end{itemize}
%
%\runtitle{Transformation $\alignS$.}
%$\alignS$ transforms a schedule $\niceSchij{}$ for nice jobs into a schedule $\alignSchij{}$ for jobs with uniform widths and aligned feasible intervals by shifting the execution interval of every job $\Job{} \in \niceJSloose$.
%\begin{itemize}
%\item $\Stime{\alignSchij{}}{\alignJob{}} \leftarrow \min\{ \alignDline{}-\w(\alignJob{}), \min_{i\geq 0} \{i\cdot w\mid i\cdot w\geq\Stime{\Schij{}}{\Job{}}\}\}$;
%\item $\Etime{\alignSchij{}}{\alignJob{}} \leftarrow \Stime{\alignSchij{}}{\alignJob{}} + \alignWidth{}$.
%\end{itemize}
%
%\runtitle{Transformation $\relaxS$.} $\relaxS$ transforms a schedule $\Sch$ into a schedule $\niceSchij{}$ for the corresponding nice jobs by moving the start and end time of every job $\Job{}$.
%
%\begin{itemize}
%\item $\Stime{\niceSchij{}}{\niceJob{}} = \min\{ \niceDline{}-\niceWidth{}, \Stime{S}{\Job{}}\}$
%\item $\Etime{\niceSchij{}}{\niceJob{}} = \Stime{\niceSchij{}}{\niceJob{}} + \niceWidth{}$.
%\end{itemize}

%By Lemma~\ref{lm:alignS} and~\ref{lm:niceload} we know that:
%
%
%\begin{lemma}
%%\label{lm:niceload}
%Let $\Jobset_{p}$ and $\niceJobsetij{p}$ denote the set of jobs $\Job{}$ with width $2^{p-1}<\Width{}\leq 2^p$ where integer $p>q$ and the nice jobs generated by $\convert$. Also we denote $\Schij{p}$ and $\niceSchij{p}$ as the schedule of $\Jobset_{p}$ and the schedule generated by $\relaxS$. 
%For any time $t$, $\Load{\niceSchij{p}}{t} \leq 2(\Load{\Schij{p}}{t} + \Load{\Schij{p}}{t - (2^{p-1}-1)} + \Load{\Schij{p}}{t + (2^{p-1}-1)})$. 
%\end{lemma}
\runtitle{\hhl{An overview of the online algorithm $\Alg$.}} 
\hhl{
Recall that the main idea of $\Alg$ is generating the algorithm for unit width jobs, $\AlgV$. 
Given input job set $\JS$, the algorithm $\AlgV$ references to a reference schedule $\R$ with input set $\JS'$ corresponding to $\JS$. 
At timeslot $t$, the algorithm $\AlgV$ assign the available job with earliest deadline at $t$ until the total load at $t$ is at least the speed of $\R$ at $t$ or there is no job left. 
The algorithm $\AlgV$ can be generalized to $\AlgUV$, an algorithm for jobs with uniform width. 
The jobs are classified by the length of feasible interval. A jobs is a tight job if its feasible interval is less than twice of its width, otherwise, it is a loose job. 
In $\AlgUV$, a tight job is executed once it is released. On the other hand, the feasible intervals of the loose jobs are modified by Procedure $\convertfi$ and the algorithm $\AlgV$ can be applied on the modified loose jobs set. 
The algorithm $\AlgUV$ can be generalized to $\Alg$. In $\Alg$ the jobs are classified by their widths such that in each class, the ratio between the maximum job width and the minimum job width is at most $2$. 
For each class, the jobs are modified by Procedure $\convertw$ such that every job has uniform width. Then, the algorithm $\AlgUV$ is applied independently on each class. 
}

\runtitle{Analysis of the online algorithm $\Alg$.} 
Now we analyze the online algorithm $\Alg$ and show that it is $O(\hhl{\lceil \log \frac{\wmax}{\wmin} \rceil})$-competitive with respect to the maximum \hhl{load}. 
%\hhl{Analysis of the online algorithm $\Alg$ with respected to the maximum power request.} 
%In the $\peak$ problem we want to minimize the maximum power request. 

%We first introduce an observation which is widely used throughout the analysis:
%\begin{observation}
%\label{ob:peak_expand}
%For two schedule $\Schij{1}$ and $\Schij{2}$, if the following relation between the loads holds 
%$\Load{\Schij{1}}{t} \leq \sum^k_{i = 1} \Load{\Schij{2}}{c_i(t)}$, where $c_i(t)$ is a function of $t$, 
%then $\p(\Schij{1})\leq k\cdot \p(\Schij{2})$. 
%\end{observation}
%
%\begin{proof}
%By definition, $\p(\Schij{1}) = \max_t \Load{\Schij{1}}{t}$. 
%By the given condition, $\p(\Schij{1}) \leq \max_t \sum^k_{i = 1} \Load{\Schij{2}}{c_i(t)} \leq \sum^k_{i=1} \max_t \Load{\Schij{2}}{c_i(t)} = \sum^k_{i=1} \p(\Schij{2}) = k \cdot \p(\Schij{2})$. 
%\end{proof}

%Recall that in Section~\ref{sec:general}, we solve the general case by generalizing the online algorithm for special input. 
%The algorithm $\AlgV$ can schedule unit-width jobs with promising performance by referencing to an arbitrary feasible online algorithm for the $\dvs$ problem. 
%By generalizing $\AlgV$, we have online algorithm~$\AlgUV$ for jobs with uniform width. By further generalizing~$\AlgUV$, we have online algorithm~$\Alg$ for jobs with arbitrary widths and arbitrary heights. 
Recall that in Sections~\ref{sec:general_unit_width} and~\ref{sec:general}, we have presented three online algorithms for different input restrictions: $\AlgV$ for unit-width jobs, $\AlgUV$ for uniform-width jobs, and $\Alg$ for arbitrary widths. Below we adapt the analysis in Section 4 to the objective function peak load. In summary, we show the following results:
\begin{itemize}
\item for unit-width job set $\Jobsetij{}$, $\p(\AlgV(\Jobsetij{})) \leq 2(e+e^2)\cdot \p(\Opt(\Jobsetij{}))$ (Theorem~\ref{thm:algV_peak})
\item for uniform-width job set $\Jobsetij{}$, $\p(\AlgUV(\Jobsetij{})) \leq (6(e+e^2)+3)\cdot \p(\Opt(\Jobsetij{}))$ (Theorem~\ref{thm:UV_peak})
\item for arbitrary-width job set $\Jobsetij{}$, $\p(\Alg(\Jobsetij{})) \leq (18(e+e^2)+9)\cdot \lceil\log \frac{\wmax}{\wmin} \rceil \cdot \p(\Opt(\Jobsetij{}))$ (Theorem~\ref{thm:alg_peak})
\end{itemize}

We first prove that the algorithm $\AlgV$ for unit-width jobs \hhl{is constant competitive} by referencing to $\newBKP$. 
Recall that for each timeslot t, $\AlgV$ schedules jobs to start at $t$ such that $\Load{\AlgV}{t}$ is at least $\Load{\newBKP}{t} = (1+e)\cdot\Load{\BKP}{t}$ or until all available jobs have been scheduled.
We prove that although $\Load{\AlgV}{t}$ might be higher than $\Load{\newBKP}{t}$, the peak of $\AlgV$ is no more than $\hhl{2(e+e^2)}$ times of the peak of the optimal. 

\begin{theorem}
\label{thm:algV_peak}
For any job set $\Jobsetij{}$ where for each job has unit width, 
$\p(\AlgV(\Jobsetij{})) \leq 2(e+e^2)\cdot \p(\Opt(\Jobsetij{}))$. 
\end{theorem}

\begin{proof}
\hhl{
Recall that in $\AlgV$, jobs are assigned in EDF manner according to the reference schedule generated by $\newBKP$. 
At each timeslot $t$, available jobs with earliest deadlines are assigned at $t$  until the sum of the jobs are at least the speed of $\newBKP$ at $t$ or there is no available jobs.
Let $\hmax(\AlgV,t)$ be the maximum height of jobs scheduled at $t$ by $\AlgV$; we set $\hmax(\AlgV, t)= 0$ if $\AlgV$ assigns no job at $t$.
}

\hhl{
We classify each timeslot $t$ into two types: 
(i) $\hmax(\AlgV,t) < \Load{\newBKP}{t}$, and (ii) $\hmax(\AlgV,t) \geq \Load{\newBKP}{t}$. 
We denote by $\I_1$ and $\I_2$ the union of all timeslots of Type (i) and (ii), respectively. 
(Notice that $\I_1$ and $\I_2$ can be empty and the union of $\I_1$ and $\I_2$ covers the entire time line.) 
We first prove that for any job set $\Jobsetij{}$ where for each job $\Job{} \in \Jobsetij{}$, $\Width{} =1$, 
$\p(\AlgV(\Jobsetij{}),\I_1) \leq 2(e+e^2)\cdot \p(\Opt(\Jobsetij{}))$; and $\p(\AlgV(\Jobsetij{}),\I_2) \leq 2 \cdot \p(\Opt(\Jobsetij{}))$. 
For every timeslot $t \in \I_1$, $\Load{\AlgV}{t} < \Load{\newBKP}{t} + \hmax(\AlgV,t) \leq 2\cdot \Load{\newBKP}{t}\leq2(1+e)\cdot\Load{\BKP}{t}$. 
By definition, let $t$ bet the timeslot where $\Load{\AlgV}{t} \geq \Load{\AlgV}{t'}$ for any other $t'$, $\p(\AlgV, \I_1) = \Load{\AlgV}{t} \leq 2(1+e)\cdot \Load{\BKP}{t}$. 
%By Lemma~\ref{lm:BKP_peak}, $\Load{\BKP}{t} \leq \max_{t} \Load{\BKP}{t}$. 
Therefore, $\p(\AlgV, \I_1)\leq 2e(1+e)\cdot\p(\Opt)$ by Observation~\ref{ob:opt_peak} and Lemma~\ref{lm:BKP_peak}. 
For every timeslot $t \in \I_2$, $\Load{\AlgV}{t} < \Load{\newBKP}{t} + \hmax(\AlgV,t) \leq 2\cdot \hmax(\AlgV,t)$. 
In the optimal schedule, the job with height $\hmax(\AlgV,t)$ has to be scheduled somewhere or the schedule is not feasible, so $\p(\Opt) \geq \hmax(\AlgV,t)$. 
Hence, $\p(\AlgV, \I_2) = \Load{\AlgV}{t} \leq 2\hmax(\AlgV,t) \leq 2\cdot \p(\Opt)$ where $t$ is the timeslot with peak power.}

%In Lemma~\ref{lem:algv_peak_I} bounds the cost of $\AlgV$ in each type of timeslots, and Theorem~\ref{thm:algV_peak} asserts that $\AlgV$ is $2(e+e^2)$-competitive. 
\hhl{Since $\I_1$ and $\I_2$ are disjoiont, $\p(\AlgV) =\max\{\p(\AlgV, \I_1), \p(\AlgV, \I_2)\}$. 
Therefore, $\p(\AlgV) = \max\{2(e+e^2)\cdot \p(\Opt), 2\cdot \p(\Opt)\} = 2(e+e^2)\cdot \p(\Opt)$.}
\end{proof}


%\begin{lemma}
%\label{lem:algv_peak_I} 
%For any job set $\Jobsetij{}$ where for each job $\Job{} \in \Jobsetij{}$, $\Width{} =1$, 
%(i) $\p(\AlgV(\Jobsetij{}),\I_1) \leq 2(e+e^2)\cdot \p(\Opt(\Jobsetij{}))$; and (ii) $\p(\AlgV(\Jobsetij{}),\I_2) \leq 2 \cdot \p(\Opt(\Jobsetij{}))$. 
%\end{lemma}
%
%\begin{proof}
%%(i) For every timeslot $t \in \I_1$, $\Load{\AlgV(\alignJobsetij{})}{t} < \Load{\BKP(\alignJobsetij{})}{t} + \hmax(\AlgV,t) \leq 2\cdot \Load{\BKP(\alignJobsetij{})}{t}$. 
%%By definition, $\cost(\AlgV(\alignJobsetij{}, \I_1)) = \max_{t\in\I_1} \Load{\AlgV(\alignJobsetij{})}{t} < 2\cdot \Load{\BKP(\alignJobsetij{})}{t}$. 
%(i) For every timeslot $t \in \I_1$, $\Load{\AlgV}{t} < \Load{\newBKP}{t} + \hmax(\AlgV,t) \leq 2\cdot \Load{\newBKP}{t}\leq2(1+e)\cdot\Load{\BKP}{t}$. 
%By definition, $\p(\AlgV, \I_1) = \max_{t\in\I_1} \Load{\AlgV}{t} < 2(1+e)\cdot \Load{\BKP}{t}$. 
%%By Lemma~\ref{lm:BKP_peak}, $\Load{\BKP}{t} \leq \max_{t} \Load{\BKP}{t}$. 
%Therefore, $\p(\AlgV, \I_1)\leq 2e(1+e)\cdot\p(\Opt)$ by Observation~\ref{ob:opt_peak} and Lemma~\ref{lm:BKP_peak}. 
%
%(ii) For every timeslot $t \in \I_2$, $\Load{\AlgV}{t} < \Load{\newBKP}{t} + \hmax(\AlgV,t) \leq 2\cdot \hmax(\AlgV,t)$. 
%In the optimal schedule, the job with height $\hmax(\AlgV,t)$ has to be scheduled somewhere or the schedule is not feasible, so $\p(\Opt) \geq \hmax(\AlgV,t)$. 
%Hence, $\p(\AlgV, \I_2) = \max_{t\in\I_2} \Load{\AlgV}{t} \leq 2\hmax(\AlgV,t) \leq 2\cdot \p(\Opt)$.
%\end{proof}


\medskip

Next, we show that $\AlgUV$ is $(6(e+e^2)+3)$-competitive (Theorem~\ref{thm:UV_peak}). 
\hhl{Recall that we classify the jobs into tight jobs and loose jobs.}
We let $\niceJobsetij{}$ denote the input set where jobs have uniform width, $\niceJStight$ denote the tight job set in $\niceJobsetij{}$ and $\niceJSloose$ denote the loose job set in $\niceJobsetij{}$. 

\hhl{For the loose jobs set $\niceJSloose$ where jobs have uniform width $\w$, we transform it to $\alignJobsetij{}$ by $\convertfi$ into jobs with release times and deadlines being at $i\cdot \w$ for certain integers $i$. 
The schedule $\AlgUV(\niceJSloose)$ is transformed from the schedule $\AlgV(\alignJobsetij{})$ by $\freeS$. 
We prove that $\AlgUV(\niceJSloose)$ is constant competitive (Lemma~\ref{lm:loose_peak}). 
For the tight jobs in $\niceJStight{}$, each job is executed once it is released. We prove that any feasible schedule for tight jobs is $3$-competitive due to the ``inflexibility'' (Lemma~\ref{lm:tight_peak}).}
%In the following we prove that the Transformation $\freeS$ does not affect the performance (Lemma~\ref{lm:nice_to_align_peak}), and the Transformation $\alignS$ does not enlarge the gap between the peak of $\AlgUV$ and the peek of $\Opt$ too much (Lemma~\ref{lem:align_to_nice_peak_2}). 
%Hence, the $\AlgUV(\niceJSloose)$ is $O(1)$-competitive (Lemma~\ref{lm:loose_peak}). 
%First we prove that any feasible schedule for tight jobs is $3$-competitive because of the ``inflexibility''. 

\begin{lemma}
\label{lm:tight_peak}
For any feasible schedule $\Schij{}$, $\p(\Schij{}(\niceJStight)) \leq 3\cdot \p(\Opt(\niceJobsetij{}))$.
\end{lemma}

\begin{proof}
We prove it by showing that even if the execution intervals of jobs are considered as the whole feasible interval, the peak is not too much larger than the peak in the optimal schedule. 

We first \emph{extend} jobs $\Job{}\in\niceJStight$ to $J^+$ as the following: $\niceRtime{} = \Rtime{}$, $\niceDline{}= \Dline{}$, $\niceWidth{}=\Dline{}-\Rtime{}$, and $\niceHeight{} = \Height{}$. 
That is, every job has its width as the length of its feasible interval. 
We denote the resulting job set by $\Jobset^+$. 
\hhl{Since} each job in $\Jobset^+$ are not shiftable, there is only one feasible schedule for $\Jobset^+$ and it is optimal. 
It is clear that $\p(\Sch(\niceJStight)) \leq \p(\Opt(\Jobset^+))$. 

Similar to Lemma~\ref{thm:cost_UV1} (i), we can bound the load at any time $t$ of $\Opt(\Jobset^+)$ by the loads of constant number of timeslots in $\Sch(\niceJStight)$. 
Consider the job $\Job{}$ corresponding to $J^+$, the execution interval of $\Job{}$ in any feasible schedule must contains either timeslot $t-(\w-1)$, $t+(\w-1)$, or $t$.  
Hence we can upper bound the load at any time $t$ in $\Opt(\Jobset^+)$ as following: $\Load{\Opt(\Jobset^+)}{t}\leq \Load{\Opt(\niceJStight)}{t-(\w-1)}+\Load{\Opt(\niceJStight)}{t+(\w-1)} + \Load{\Opt(\niceJStight)}{t}$.
Hence, $\p(\Sch(\niceJStight)) \leq\p(\Opt(\Jobset^+)) \leq 3\cdot \p(\Opt(\niceJSloose))$.
\end{proof}

%Recall that for the loose jobs set $\niceJSloose{}$ where jobs have uniform width $\w$, we transform it to $\alignJobsetij{}$ by $\convertfi$ into jobs with release times and deadlines being at $i\cdot \w$ for certain integers $i$. 
%The schedule $\AlgUV(\niceJSloose)$ is transformed from the schedule $\AlgV(\alignJobsetij{})$ by $\freeS$. 
%In the following we prove that the Transformation $\freeS$ does not affect the performance (Lemma~\ref{lm:nice_to_align_peak}), and the Transformation $\alignS$ does not enlarge the gap between the peak of $\AlgUV$ and the peek of $\Opt$ too much (Lemma~\ref{lem:align_to_nice_peak_2}). 
%Hence, the $\AlgUV(\niceJSloose)$ is $O(1)$-competitive (Lemma~\ref{lm:loose_peak}). 

%\begin{lemma}
%\label{lm:nice_to_align_peak}
%Given $\alignSchij{}$, consider the $\niceSchij{}$ generated by $\freeS$, $\p(\niceSchij{}) = \p(\alignSchij{})$. 
%\end{lemma}
%
%\begin{proof}
%It is easy to see that $\Load{\niceSchij{}}{t} = \Load{\alignSchij{}}{t}$ for all $t$. Hence $\p(\niceSchij{}) = \p(\alignSchij{})$.
%\end{proof}
%
%According to Lemma~\ref{thm:align_load}, we know that for any schedule $\niceSchij{}$ for $\niceJSloose$ and the schedule $\alignSchij{}$ for $\alignJobsetij{}$ constructed by $\alignS$, 
%at any timeslot $t$, $\Load{\alignSchij{}}{t} \leq \Load{\niceSchij{}}{t} + \Load{\niceSchij{}}{t-(\w-1)} + \Load{\niceSchij{}}{t+(\w-1)}$.
%Therefore we have the following lemma:
%%The proof is exactly the same as the proof of Lemma~\ref{lm:alignS}. 
%
%
%%\begin{observation}
%%$\Load{\alignSchij{}}{t} \leq \Load{\niceSchij{}}{t} + \Load{\niceSchij{}}{t-(\w-1)} + \Load{\niceSchij{}}{t+ (\w-1)}$. 
%%\end{observation}
%%
%%\begin{proof}
%%\end{proof}
%
%%\begin{lemma}
%%\label{lem:align_to_nice_peak}
%%Given $\niceSchij{}$ and using $\alignS$ to generate $\alignSchij{}$, $\p(\alignSchij{}) \leq 3\cdot \p(\niceSchij{})$. 
%%\end{lemma}
%%
%%\begin{proof}
%%By definition, $\p(\alignSchij{}) = \max_t \Load{\alignSchij{}}{t}$. 
%%By Observation~\ref{lm:alignS_2} and Observation~\ref{ob:peak_expand}, $\p(\alignSchij{}) \leq \max_t (\Load{\alignSchij{}}{t} \leq \Load{\niceSchij{}}{t} + \Load{\niceSchij{}}{t-(\w-1)} + \Load{\niceSchij{}}{t+(\w-1)})\\ \leq 3 \cdot \p(\niceSchij{})$. 
%%\end{proof}
%
%\begin{lemma}
%\label{lem:align_to_nice_peak_2}
%Given a schedule $\niceSchij{}$ for a set of loose jobs $\niceJSloose$ with uniform width and the schedule $\alignSchij{}$ generated by $\alignS$ for the corresponding $\alignJobsetij{}$ generated by Procedure $\convertfi$, $\p(\Opt(\alignJobsetij{})) \leq 3\cdot \p(\Opt(\niceJSloose))$. 
%\end{lemma}
%
%\begin{proof}
%By definition, $\p(\alignSchij{}) = \max_t \Load{\alignSchij{}}{t}$. 
%By Lemma~\ref{thm:align_load} and Observation~\ref{ob:peak_expand}, $\p(\alignSchij{}) \leq \max_t (\Load{\alignSchij{}}{t} \leq \Load{\niceSchij{}}{t} + \Load{\niceSchij{}}{t-(\w-1)} + \Load{\niceSchij{}}{t+(\w-1)})\\ \leq 3 \cdot \p(\niceSchij{})$. 
%Given $\Opt(\niceJSloose)$, there exists a schedule $\Sch(\alignJobsetij{})$ generated by $\alignS$. 
%Therefore, $\p(\Sch(\alignJobsetij{})) \leq 3\cdot\p(\Opt(\niceJSloose))$. 
%Hence $\p(\Opt(\alignJobsetij{})) \leq \p(\Sch(\alignJobsetij{})) \leq 3\cdot\p(\Opt(\niceJSloose))$. 
%\end{proof}

\begin{lemma}
\label{lm:loose_peak}
For loose jobs set $\niceJSloose$ where jobs have uniform width, $\p(\AlgUV(\niceJSloose)) \leq 6(e+e^2) \cdot \p(\Opt(\niceJobsetij{}))$. 
\end{lemma}

\begin{proof}

%By Observation~\ref{lm:alignS_2}, $\Load{\alignSchij{}}{t} \leq \Load{\niceSchij{}}{t} + \Load{\niceSchij{}}{t-(\w-1)} + \Load{\niceSchij{}}{t+(\w-1)}$. 
According to $\AlgUV$, the job set $\niceJSloose$ is transformed into a job set $\alignJobsetij{}$ by $\convertfi$ and $\AlgV$ is run on~$\alignJobsetij{}$. 
Then, the schedule $\AlgV(\alignJobsetij{})$ is transformed to a schedule of $\niceJSloose$ by Transformation $\freeS$. 
\hhl{Hence, $\p(\AlgUV(\niceJSloose)) \leq \p(\AlgV(\alignJobsetij{}))\leq 2(e+e^2)\cdot \p(\Opt(\alignJobsetij{}))$. The inequality is by Theorem~\ref{thm:algV_peak}.}

\hhl{
Now we prove that after $\convertfi$, $\p(\Opt(\alignJobsetij{})) \leq 3\cdot \p(\Opt(\niceJSloose))$. 
%By definition, $\p(\alignSchij{}) = \Load{\alignSchij{}}{t}$ where $t$ is the timeslot having peak load. 
Given the optimal schedule~$\Opt(\niceJSloose)$, let $\alignSchij{}$ be the schedule generated by $\alignS$ for the job set $\alignJobsetij{}$ corresponding to $\niceJSloose$.
Let $t$ be the timeslot with the peak load in $\alignSchij{}$, by Lemma~\ref{thm:align_load}, $\p(\alignSchij{}) = \Load{\alignSchij{}}{t} \leq \Load{\Opt(\niceJSloose)}{t} + \Load{\Opt(\niceJSloose)}{t-(\w-1)} + \Load{\Opt(\niceJSloose)}{t+(\w-1)}\leq 3 \cdot \p(\Opt(\niceJSloose))$. 
Therefore, $\p(\Opt(\alignJobsetij{})) \leq \p(\Sch(\alignJobsetij{})) \leq 3\cdot\p(\Opt(\niceJSloose))$. 
}

\hhl{In summary, $\p(\AlgUV(\niceJSloose))\leq 2(e+e^2)\cdot \p(\Opt(\alignJobsetij{}))\leq 6(e+e^2) \cdot \p(\Opt(\niceJSloose))$}
%
%In summary, $\p(\Opt(\alignJobsetij{})) \leq 3\cdot \p(\Opt(\niceJSloose))$. 
%Hence, $\p(\AlgUV(\niceJSloose)) \leq 6(e+e^2) \cdot \p(\Opt(\niceJobsetij{}))$. 
\end{proof}

Now we are ready to prove that the algorithm $\AlgUV$ performs well when the tight jobs and loose jobs are considered together: 

\begin{theorem}
\label{thm:UV_peak}
\hhl{For any jobs set $\niceJobsetij{}$ where jobs have uniform width,} $\p(\AlgUV(\niceJobsetij{})) \leq (6(e+e^2)+\hhl{3})\cdot \p(\Opt(\niceJobsetij{}))$. 
\end{theorem}

\begin{proof}
By definition, $\p(\AlgUV(\niceJobsetij{})) \leq \p(\AlgUV(\niceJStight)) + \p(\AlgUV(\niceJSloose))$. 
By Lemma~\ref{lm:tight_peak} and~\ref{lm:loose_peak}, $\p(\AlgUV(\niceJobsetij{})) \leq 3\cdot\p(\Opt(\niceJobsetij{})) + 6(e+e^2)\cdot \p(\Opt(\niceJobsetij{})) = {(6(e+e^2)+3)}\cdot \p(\Opt(\niceJobsetij{}))$. 
\end{proof}

\medskip

Finally we can bound the competitive ratio of $\Alg$. 

%We show that $\shrinkS$ does not increase the peak in Lemma~\ref{lm:JS_to_nice_peak}. 
%On the other hand, we show that the effect on considering jobs as nice jobs is bounded (Lemma~\ref{lm:nice_to_JS_opt_peak}). 
%%\begin{lemma}
%%\label{lm:niceload_2}
%Let $\Jobset_{p}$ and $\niceJobsetij{p}$ denote the set of jobs in class $\classij{p}$ and the nice jobs generated by $\convert$. Also we denote $\Schij{p}$ and $\niceSchij{p}$ as the schedule of $\Jobset_{p}$ and the schedule generated by $\relaxS$. 
%According to Lemma~\ref{thm:relax_load}, we know that
%for any time $t$, $\Load{\niceSchij{p}}{t} \leq \Load{\Schij{p}}{t} + \Load{\Schij{p}}{t - (2^{p-1}-1)} + \Load{\Schij{p}}{t + (2^{p-1}-1)}$. 
%%\end{lemma}
%Hence we have the following lemma:
%
%\begin{lemma}
%\label{lm:nice_to_JS_peak}
%Given $\Schij{p}$ and $\niceSchij{p}$ generated by $\relaxS$, $\p(\niceSchij{p}) \leq 3\cdot \p(\Schij{p})$
%\end{lemma}
%
%\begin{proof}
%By Lemma~\ref{thm:relax_load} and Observation~\ref{ob:peak_expand}, $\p(\niceSchij{p}) = \max_t \Load{\niceSchij{p}}{t} \leq \max_t (\Load{\Schij{p}}{t} + \Load{\Schij{p}}{t - (2^{p-1}-1)} + \Load{\Schij{p}}{t + (2^{p-1}-1)}) \leq 3\cdot \p(\Schij{p})$. 
%\end{proof}
%
%\begin{lemma}
%\label{lm:nice_to_JS_opt_peak}
%Consider any job set $\Jobsetij{}$, its corresponding $\niceJobsetij{}$ and the corresponding job set of each class $\Jobsetij{p}$ and $\niceJobsetij{p}$, $\p(\Opt(\niceJobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{}))$.
%\end{lemma}
%
%\begin{proof}
%Given $\Opt(\Jobsetij{p})$, there exists schedule $\Sch(\niceJobsetij{p})$ generated by $\relaxS$. 
%By Lemma~\ref{lm:nice_to_JS_peak}, $\p(\Sch(\niceJobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{p}))$. 
%Hence, $\p(\Opt(\niceJobsetij{p})) \leq \p(\Sch(\niceJobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{}))$.
%\end{proof}
%
%\begin{lemma}
%\label{lm:JS_to_nice_peak}
%Using $\shrinkS$, $\p(\Schij{p}) \leq \p(\niceSchij{p})$
%\end{lemma}
%
%\begin{proof}
%It can be easily seen that for all $t$, $\Load{\Schij{p}}{t} \leq \Load{\niceSchij{p}}{t}$. Hence $\p(\Schij{p}) \leq \p(\niceSchij{p})$.
%\end{proof}
%
%The following theorem asserts that $\Alg$ is {$O(\hhl{\lceil\log \frac{\wmax}{\wmin} \rceil})$}-competitive. 

\begin{theorem}
\label{thm:alg_peak}
For any job set $\Jobsetij{}$, {$\p(\Alg(\Jobsetij{})) \leq {(\hhl{18(e+e^2)+9})}\cdot \lceil\log \frac{\wmax}{\wmin} \rceil \cdot \p(\Opt(\Jobsetij{}))$}.
\end{theorem}

\begin{proof}
\hhl{Recall that $\Alg(\Jobset)$ partition jobs into subsets $\Jobsetij{p}$ such that in each $\Jobsetij{p}$ jobs have bounded widths. 
For each $\Jobsetij{p}$, it is transformed into $\niceJobsetij{p}$ and $\AlgUV$ is applied independently on each class. 
Then,~$\AlgUV(\niceJobsetij{p})$ is transformed into a schedule for $\Jobsetij{p}$ by Transformation $\shrinkS$. 
%Then, $\Alg(\Jobsetij{p}) = \AlgUV(\niceJobsetij{p})$ and Transformation $\shrinkS$ is applied. 
By Observation~\ref{thm:shrink_feasible}, $\Load{\Alg(\Jobsetij{p})}{t} \leq \Load{\AlgUV(\niceJobsetij{p})}{t}$. 
Hence, $\Load{\Alg(\Jobset)}{t} = \sum_p \Load{\Alg(\Jobsetij{p})}{t} \leq \sum_p \Load{\AlgUV(\niceJobsetij{p})}{t}$ for all~$t$. 
}

\hhl{
Consider the timeslot $t$ with peak load in $\Alg(\Jobsetij{})$, $p(\Alg(\Jobsetij{})) = \Load{\Alg(\Jobsetij{})}{t} \leq\sum_p \Load{\AlgUV(\niceJobsetij{p})}{t} \leq \sum_p \p(\AlgUV(\niceJobsetij{p}))$
}
%By definition, $\p(\Alg(\Jobsetij{})) = \max_t \Load{\Alg(\Jobsetij{})}{t} \leq \max_t \Load{\Alg(\niceJobsetij{})}{t} = \max_t \sum^{\lceil\log \frac{\wmax}{\wmin}\rceil}_{p=1} \Load{\AlgUV(\niceJobsetij{p})}{t}$.
%By shuffling the terms, $\p(\Alg(\Jobsetij{})) \leq \sum^{\lceil\log \frac{\wmax}{\wmin}\rceil}_{p=1}\p(\AlgUV(\niceJobsetij{p}))$. 
By Theorem~\ref{thm:UV_peak}, $\p(\Alg(\Jobsetij{})) \leq \sum_p {(6(e+e^2)+3)}\cdot \p(\Opt(\niceJobsetij{p}))$. 

\hhl{
Now we prove that $\p(\Opt(\niceJobsetij{p})) \leq 3 \cdot \p(\Opt(\Jobsetij{}))$. 
Consider the job set $\Jobsetij{p}$ and the corresponding~$\niceJobsetij{p}$ generated by $\convert$. 
Given $\Opt(\Jobsetij{p})$, there exists schedule $\Sch(\niceJobsetij{p})$ generated by Transformation $\relaxS$. 
Let $t$ be the timeslot with peak load in $\Sch(\niceJobsetij{p})$, by Lemma~\ref{thm:relax_load}, $\p(\Sch(\niceJobsetij{p}))= \Load{\niceSchij{p}}{t} \leq \Load{\Opt(\Jobsetij{p})}{t} + \Load{\Opt(\Jobsetij{p})}{t - (2^{p-1}-1)} + \Load{\Opt(\Jobsetij{p})}{t + (2^{p-1}-1)} \leq 3\cdot \p(\Opt(\Jobsetij{p}))$. 
Hence, $\p(\Opt(\niceJobsetij{p})) \leq \p(\Sch(\niceJobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{p})) \leq 3\cdot \p(\Opt(\Jobsetij{}))$.
}

In summary, $\p(\Alg(\Jobsetij{}))\leq \sum_p {(6(e+e^2)+3)}\cdot \p(\Opt(\niceJobsetij{p})) \leq \sum_p {(6(e+e^2)+3)}\cdot 3\cdot \p(\Opt(\Jobsetij{})) \leq {(18(e+e^2)+9)}\cdot \lceil\log \frac{\wmax}{\wmin}\rceil \cdot \p(\Opt(\Jobsetij{}))$. 
\end{proof}

\bigskip

%\begin{lemma}
%%\label{lm:alignS}
%Consider any schedule $\Schij{}$ for $\JSloose$ and the schedule $\alignSchij{}$ for $\alignJobsetij{}$ constructed by $\alignS$. 
%At any timeslot $t$, $\Load{\alignSchij{}}{t} \leq \Load{\Schij{}}{t} + \Load{\Schij{}}{t-(\w-1)} + \Load{\Schij{}}{t+(\w-1)}$.
%\end{lemma}
%
%\begin{lemma}
%%\label{lm:niceload}
%Let $\Jobset_{p,q}$ and $\niceJobsetij{p,q}$ denote the set of jobs in class $\classij{p,q}$ and the nice jobs generated by $\convert$. Also we denote $\Schij{p,q}$ and $\niceSchij{p,q}$ as the schedule of $\Jobset_{p,q}$ and the schedule generated by $\relaxS$. 
%For any time $t$, $\Load{\niceSchij{p,q}}{t} \leq 2(\Load{\Schij{p,q}}{t} + \Load{\Schij{p,q}}{t - (2^{p-1}-1)} + \Load{\Schij{p,q}}{t + (2^{p-1}-1)})$. 
%\end{lemma}

\runtitle{The non-preemptive Machine Minimization problem. }
The Machine Minimization problem is as follows. 
The inputs are a set of jobs~$\Job{}$ with processing times~$\Work{}$, release times~$\Rtime{}$, and deadlines~$\Dline{}$ and infinite number of machines. 
Each machine can serve only one job at a time. 
Each job has to be scheduled on a machine such that in its execution interval (which is in the interval between its start time and end time) there is no other job assigned on the same machine. 
The goal is to minimize the number of used machines.

The Machine Minimization problem can be seen as a special case of the $\peak$ problem by considering the processing time as the time duration of the job. 
In the Machine Minimization problem, the jobs have no power request. 
Hence we can reduce an input set $\Jobsetij{M}$ of the machine minimization problem to an input set $\Jobsetij{D}$ of the $\peak$ problem as follows. 
For every job $\Job{}\in \Jobsetij{M}$, there is a corresponding job $\alignJob{} \in \Jobsetij{D}$ with $\alignWidth{} \leftarrow \Work{}$, $\alignHeight{} \leftarrow 1$, $\alignRtime{} \leftarrow \Rtime{}$ and $\alignDline{} \leftarrow \Dline{}$.
By Theorem~\ref{thm:alg_peak}, we prove that there exists an asymptotically optimal online algorithm for the Machine Minimization problem.


\section{The interval graph approach on the $\peak$ problem}
\label{sec:other_fpt}
%\note{machine minimization, min peak, interval coloring?}

In Section~\ref{sec:exact_fpt}, we introduced an exact algorithm $\AlgE$ using the \emph{linear clique arrangement} property of the interval graphs. 
The linear property of the consecutive clique arrangement of interval graphs gives
a direction to design a dynamic programming algorithm, which breaks down a problem
into overlapped subproblems until the subproblems are simple enough to be solved. 
\hhl{In the following of this section, we show that the $\AlgE$ can be used to solve the $\peak$ problem by changing the objective function.} 

\runtitle{Algorithm $\AlgE_{peak}$ for the $\peak$ problem (also see Section~\ref{sec:exact_fpt}).}
The jobs are considered as time intervals and the time horizon is chopped into ``windows''. 
%We first transform the input job set~$\Jobsetij{}$ to an interval graph, and obtain the maximal cliques~$C_i$ for $1 \leq i \leq k$ and the corresponding windows~$\win_i$.
The algorithm visits all windows accordingly from the left to the right. 
In Stage $i$, the $i$-th window is visited and the algorithm maintains a candidate set of schedules for the visited windows that no optimal solution is deleted from the set. 
In each Stage $i$, the algorithm consists of three procedures: ListConfigurations, ConcatenateTables and FilterTable. 

The ListConfigurations procedure lists all possible configurations (i.e., execution segments) of the jobs in $C_i$ within $\win_i$. The invalid configurations will be deleted. 
The valid configurations together with \textit{the peak load within $\win_i$} will be stored in a table. 

The ConcatenateTables procedure concatenates the configurations in the current window $\win_i$ and the configurations in the windows which have been seen so far. If the execution interval after concatenation is not valid, it is deleted from the table. \textit{The peak load of the new configuration is simply the maximum among the peaks of the two concatenated configurations.} 

The FilterTable procedure filters non-optimal configurations. The idea is, given a configuration of the jobs in $C_i$, there must be a best decision of the jobs in $\bigcup^{i-1}_{k=1} C_k\setminus C_i$ which has minimum \textit{peak load} within the intervals $[0,b_{i+1})$, where $b_{i+1}$ is the right boundary of the window $\win_i$. 
For each configuration, we only keep the (partial) schedule with the minimum \textit{peak load}. 

After processing all the windows, the schedule with minimum \textit{peak load} can be found in the final table. 

%In this section, we show that by changing the objective function in $\AlgE$, we can use similar idea to solve other demand response management problems with respect to different objective functions. In the following we show how to solve the $\peak$ problem.
%
%
%
%We start with $\Tl$ containing the only configuration, which sets $\stime_0(\Job{j}) = \bound_1$ and $\etime_0(\Job{j}) = \bound_1 + 1$ for all jobs $\Job{j}$.
%That is, the configuration treats all the jobs to be not yet executed.
%Then we visit the windows from the left to the right.
%
%\noindent
%\textbf{\emph{ListConfigurations:}}
%For window~$\win_i$ and jobs in $C_i$, we construct $\Tr$ storing all configurations of $\Job{j} \in C_i$.
%We enumerate all $\stime_i(\Job{j}) \in \win_i$ and $\etime_i(\Job{j}) \in \win_i$ for each job $\Job{j} \in C_i$, list all the combinations of all the jobs~$\Job{j}$ with all of its start times and end times, and store the results in $\Tr$ in the way that one row is for one configuration $\config_i(C_i)$.
%In another words, $\Tr$ stores all the combinations of execution segments in $\win_i$ for all jobs $\Job{j} \in C_i$.
%Note that the jobs with release time later than $\win_i$ are considered to execute after $\win_i$ and the jobs with deadline earlier than $\win_i$ are considered to execute before $\win_i$.
%For each configuration~$\config_i(C_i)$, we also store the maximum power request within window $\win_i$ together.
%We also check each of the configurations and delete those invalid ones.
%
%\noindent
%\textbf{\emph{ConcatenateTables:}}
%We then concatenate compatible configurations in $\Tl$ and $\Tr$. 
%The resulting table is the new $\Tl$.
%More specifically, for each configuration~$\configL(C)$ in $\Tl$ and each configuration~$\configR(C)$ in $\Tr$, we concatenate $\configL(C)$ and $\configR(C)$ if they are compatible, and store the result to a new row in $\Tl$.
%For each configuration after combining, we stop the maximum power request by then. 
%We also check each of the configurations in the new $\Tl$ and delete those invalid ones.
%
%\noindent
%\textbf{\emph{FilterTable:}}
%After concatenation, we filter non-optimal configurations.
%We classify all the configurations in $\Tl$ into groups such that the configurations in a group are identical and no two configurations from different groups are identical.
%For each group, we only leave the configuration with the minimum maximum power request (choosing anyone to break tie if any) and remove the others in the group.
%In the current $\Tl$, no two configurations are identical.
%
%After processing all windows, the only configuration in the final $\Tl$ is returned as the solution. 
%%Algorithm~\ref{alg:fpt} is the pseudocode of this algorithm.
%

%In the following of this section, we show that the $\AlgE$ can be used to solve other demand response management problems by changing the objective function.
%
%%\subsection{Minimizing the peak power request}
%To solve the $\peak$ problem, we modify the algorithm $\AlgE$ as follows. 
%Recall that in Stage $i$, in the original ListConfigurations procedure, each valid configuration will be stored in the table together with their cost. 
%We store the valid configurations together with the peak power request instead of the total cost. 
%In the ConcatenateTables procedure, the peak power request of the new configuration is the bigger one of the two concatenated configurations. 
%In the FilterTable procedure, we keep the partial schedule with minimum peak power request for each given configurations of jobs in $C_i$.


It can be seen that we list all possible configurations. 
A configuration is deleted only when it is invalid or it is identical to another configuration with lower peak \hhl{peak}.
Hence in the end we get an optimal schedule.
It also shows that the $\peak$ problem is fixed parameter tractable with respect to the maximum width of jobs and the maximum number of overlapped feasible intervals, and the maximum length of windows.

%\begin{corollary}
%The $\peak$ problem is fixed parameter tractable with respect to the maximum width of jobs, the maximum number of overlapped feasible intervals, and the maximum length of windows.
%\end{corollary}

\begin{corollary}
The $\peak$ problem is fixed parameter tractable with respect to the maximum width of jobs, and the maximum number of overlapped feasible intervals.
\end{corollary}

%\subsection{Minimizing the total cost with limited power}
%In this section we consider the $\grid$ problem with power limit $L$. 
%More formally, the aim is to find a schedule which feasibly schedule all jobs such that for every timeslot, the power request is at most $L$ and the total cost is minimized. 
%
%\runtitle{The $\limited$ problem.}
%The input of the $\limited$ problem is a set of jobs where each job has a power request, a time duration, and a feasible intervals in which the job can be scheduled. Moreover, there is a power limit $L$ such that the total power request at any timeslot cannot be more than $L$. 
%The goal is to feasibly serve all jobs without preemption such that for all timeslot $t$, $\load{}{t}\leq L$ and the total cost is minimized. 
%
%
%To solve the $\limited$ problem, we modify the algorithm $\AlgE$ by redefining the ``valid'' configuration. 
%Previously the validity of configuration was only about the consistency of the execution segments; now we also consider a configuration with load at some timeslot bigger than $L$ as invalid. 
%The other parts of the algorithm $\AlgE$ remain the same. 
%%In the ListConfigurations procedure, each valid configuration will be stored in the table together with their cost. 
%%We store the valid configurations together with the peak power request instead of the total cost. 
%%In the ConcatenateTables procedure, the peak power request of the new configuration is the bigger one of the two concatenated configurations. 
%%In the FilterTable procedure, we keep the partial schedule with minimum peak power request for each given configurations of jobs in $C_i$.
%
%%\runtitle{The $\grid$ problem with limited power constraint.} 
%%So far in this thesis, we consider the smart grid scheduling problems with unlimited power supply. 
%%Which means we can have arbitrarily high power request at any timeslot. 
%%However, in real world setting the power generator might have limited ability so there is a maximum power supply. 
%%The schedule should have load at any time lower than the power limit. 
%
%It is clear that we list all possible configurations. 
%A configuration is deleted only when it is invalid, it has some timeslots with load more than $L$ or it is identical to another configuration with lower cost
%Hence in the end we get an optimal schedule and in the schedule each timeslot has load at most $L$.
%
%\begin{corollary}
%The $\limited$ problem is fixed parameter tractable with respect to the maximum width of jobs, the maximum number of overlapped feasible intervals, and the maximum length of windows.
%\end{corollary}
%
%\begin{corollary}
%The $\limited$ problem is fixed parameter tractable with respect to the maximum width of jobs, and the maximum number of overlapped feasible intervals.
%\end{corollary}



==> special.tex <==
\section{Special cases}
\label{sec:special}

\subsection{Unit height - online algorithms}
\label{sec:horizontal}

In this section we focus on unit-height jobs and consider two special cases of the width.
We first consider jobs with unit-height and unit-width (Section~\ref{sec:special_unit})
and secondly consider jobs with agreeable deadlines (Section~\ref{sec:horizontal_agreeable}).
Note that the results in Section~\ref{sec:general_uniform} are applicable to
unit-height unit-width jobs but we can improve the competitive ratio further.

To ease the discussion, we refine a notation we defined before.
For any algorithm~$\Alg$ for a job set $\JS$ and a time interval $\I$,
we denote by $\Alg(\JS,\I)$ the schedule of $\Alg$ on $\JS$ over the time interval $\I$.


\subsubsection{Framework}
\label{sec:horizontal_framework}

% \pw{[PW: to be polished - by PW]}
The main idea of the analysis is to 
make reference to the online algorithm $\AVR$
and consider two types of intervals,
$\IL{1}$ where the average load is higher than~$1$ and
$\IS{1}$ where the average load is at most $1$.
For the former, we show that we can base on the competitive ratio of $\AVR$ directly;
for the latter, our load could be much higher than that of $\AVR$ and
in such case, we compare directly to the optimal algorithm.
Combining the two cases, we derive our main theorem.

\begin{lemma}
\label{thm:ibig}
Given a job set $\JS$ with $\avg(t) >1$ $\forall t$, if we have an algorithm $\Alg$ such that there exists a constant $c$, $\load(t) \leq c\lceil \avg(t)\rceil$  $\forall t$, then $\cost(\Alg(\JS))\leq \frac{(4c\alpha)^\alpha}{2}\cdot \cost(\Opt(\JS))$. 
\end{lemma}

\begin{proof}
% \pw{[PW: to be filled in by AL/HL.]}

We prove the lemma by comparing $\load(\Alg, t)$ to $\load(\AVR, t)$ for each timeslot $t$.
The assumption of $\Alg$ means that $\load(\Alg, t) \leq c\lceil\avg(t)\rceil \leq 2c\cdot\avg(t)$ 
since $\avg(t) >1$. 
By definition, $\cost(\Alg(\JS)) = \sum_t \load(\Alg, t) \leq \sum_t (2c)^\alpha\cdot\avg(t))^\alpha$. 
Recall that $\load(\AVR, t)  = \avg(t)$ for each $t$. 
Hence, by Corollary~\ref{thm:AVR},
$\cost(\Alg(\JS))\leq (2c)^\alpha\cdot\cost(\AVR(\JS)) \leq \frac{(4c\alpha)^\alpha}{2}\cdot\cost(\Opt(\JS))$.
\end{proof}

\begin{theorem}
\label{thm:horizontal_framework}
Suppose we have an algorithm $\Alg$ for a job set $\JS$ such that (i) $\load(t) \leq c\cdot \lceil \avg(t)\rceil$ for all $t\in \IL{1}$, 
and (ii) $\load(t) \leq c'$ for all $t\in \IS{1}$. 
Then we have $\cost(\Alg(\JS))\leq (\frac{(4c\alpha)^\alpha}{2}+c'^\alpha)\cdot cost(\Opt(\JS))$.
\end{theorem}


\begin{proof}
% \pw{[PW: to be filled in by AL/HL.
% Use $\cost(\AVR(\JS,\IL{1}))$ and $\cost(\AVR(\JS,\IS{1}))$
% % Consider using $\AVR|_{\IL{1}}$ and $\AVR|_{\IS{1}}$
% ]}
% 
% \hhl{
By the same argument as Lemma~\ref{thm:ibig}, we can show that 
$\cost(\Alg(\JS,\IL{1}))\leq (2c)^\alpha\cdot\cost(\AVR(\JS,\IL{1}))\leq (2c)^\alpha\cdot\cost(\AVR(\JS)) \leq \frac{(4c\alpha)^\alpha}{2}\cdot\cost(\Opt(\JS))$.
% }
% \hhl{
On the other hand, % let $\JS_{\leq 1}$ be the set of jobs available in $\I_{\leq 1}$.
% $\cost(\Alg(\JS,\IS{1}))\leq \sum_{J\in\JS_{\leq 1}} \w(J)\cdot c'^\alpha$. 
$\cost(\Alg(\JS,\IS{1}))\leq \sum_{J:J \text{ is available in } \I_{\leq 1}} \w(J)\cdot c'^\alpha$. 
By convexity, $\cost(\Opt(\JS)) \geq \sum_{J\in\JS} \w(J)\cdot \h(J)^\alpha \geq \sum_{J\in\JS} \w(J)$. 
Hence, $\cost(\Alg(\JS, \IS{1})) \leq c'^\alpha\cdot\cost(\Opt(\JS))$.
% }

% \hhl{% By adding up $\cost(\Alg(\JS, \IL{1}))$ and $\cost(\Alg(\JS,\IS{1}))$, 
Adding up the two cost,
we have $\cost(\Alg(\JS)) 
= \cost(\Alg(\JS, \IL{1})) + \cost(\Alg(\JS, \IS{1})) 
\leq (\frac{(4c\alpha)^\alpha}{2}+c'^\alpha)\cdot\cost(\Opt(\JS))$
and the theorem follows.
% }
\end{proof}

\subsubsection{Unit-height and unit-width}
\label{sec:special_unit}

In this section we consider job sets where all jobs have unit-height and unit-width,
i.e., $\w(J) = 1$ and $\h(J) = 1$  $\forall J$.
We describe the algorithm $\AlgOne$ for this case.

\runtitle{Algorithm $\AlgOne$.}
% The algorithm takes a job set $\JS$ as input where all jobs have unit-height and unit-width.
At any time $t$, 
choose $\lceil \avg(t) \rceil$ jobs according to the EDF rule 
and schedule them to start at $t$.
If there are fewer jobs available, schedule all available jobs.

The following theorem asserts that the algorithm gives feasible schedule 
and states its competitive ratio.

\begin{theorem}
\label{thm:alg_unit}
(i) The schedule constructed by Algorithm~$\AlgOne$ is feasible.
(ii) Algorithm~$\AlgOne$ is $(\frac{(4\alpha)^\alpha}{2}+1)$-competitive.
\end{theorem}

\begin{proof}
% \pw{[PW: to be filled in by AL/HL.
% (ii) Simply saying load is at most ceiling of avg is not sufficient, need to relate to that the jobs are unit height and hence $c'=1$.]}
% 
(i) The feasibility can be proved by comparing to $\AVR$.
At any time $t$, the total work done by $\AVR$ in interval $[0, t)$ is $\sum_{t'<t}\avg(t')$. 
On the other hand, the total work done by $\AlgOne$ in the same interval is 
$\sum_{t'<t}\lceil\avg(t)\rceil \geq \sum_{t'<t} \avg(t)$ 
if there are enough available jobs in this interval. 
If the number of available jobs is less than  $\sum_{t'<t}\lceil\avg(t)\rceil$, 
$\AlgOne$ will execute all these jobs. 
The work done by $\AlgOne$ within interval $[0,t)$ is at least %\pw{at least (???)} 
the work done by $\AVR$ in both cases. 
Hence, $\AlgOne$ is feasible since $\AVR$ is feasible.

(ii) We note that $\load(\AlgOne,t) \leq \lceil\avg(t)\rceil$.
To use Theorem~\ref{thm:horizontal_framework}, 
we can set $c'=1$ for $t\in\IS{1}$ by the definition of $\IS{1}$.
Furthermore, we can set $c=1$ for $t\in\IL{1}$.
% Then the theorem follows.
% For $t\in\IL{1}$, $\load(\AlgOne, t) = \lceil\avg(t)\rceil$. For $t\in\IS{1}$, $\load(\AlgOne, t)\leq 1$ since each job has unit height. 
% By Theorem~\ref{thm:horizontal_framework}, the ratio can be found by letting $c=1$ and $c'=1$.
\end{proof}

\subsubsection{Unit-height, arbitrary width and agreeable deadlines}
\label{sec:horizontal_agreeable}

In this section we consider jobs with agreeable deadlines.
We first note that simply scheduling $\lceil \avg(t) \rceil$ number of jobs may not
return a feasible schedule.

\begin{example}
Consider four jobs each job $J$ with $\rel(J)=0$, $\dl(J)=5$, $\h(J)=1$, $\w(J)=3$.
Note that $\avg(t) = 2.4$ for all $t$.
If we schedule at most $\lceil \avg(t) \rceil = 3$ jobs at any time, we can complete three jobs but the remaining job cannot be completed.
To schedule all jobs feasibly, we need at least two timeslots where all jobs are being executed.
\end{example}

To schedule these jobs, we first observe in Lemma~\ref{thm:horizontal_density} that for a set of jobs with total densities at most~$1$, it is feasible to schedule them such that the load at any time is at most~$1$.
Roughly speaking, we consider jobs in the order of release, and hence in EDF manner since the jobs have agreeable deadlines.
We keep the current ending time of all jobs that have been considered.
As a new job is released, if its release time is earlier than the current ending time,
we set its start time to the current ending time (and increase the current ending time by the width of the new job);
otherwise, we set its start time to be its release time.
Lemma~\ref{thm:horizontal_density} asserts that such scheduling is feasible
and maintains the load at any time to be at most~$1$.

Using this observation, we then partition the jobs into ``queues'' each of which has sum of densities at most~$1$.
Each queue $\queue_i$ is scheduled independently
and the resulting schedule is to ``stack up'' all these schedules.
The queues are formed in a Next-Fit manner:
(i) the current queue $\queue_q$ is kept ``open'' and a newly arrived job is added to the current queue if including it makes the total densities stays at most $1$;
(ii) otherwise, the current queue is ``closed'' and a new queue $\queue_{q+1}$ is created as open.

\begin{lemma}
\label{thm:horizontal_density}
Given any set of jobs of unit-height, arbitrary-width and agreeable deadlines.
If the sum of densities of all these jobs is at most~$1$,
then it is feasible to schedule all of them using a maximum load~$1$ at any time.
\end{lemma}

\begin{proof}
% \pw{[PW: to be filled in by AL/HL.]}
Suppose there are $k$ jobs $J_1, J_2, \cdots, J_k$ such that $\sum_{1 \leq i \leq k} \den(J_i)\leq 1$. 
Without loss of generality, we assume that $\dl(J_i) \leq \dl(J_j)$ and $\rel(J_i)\leq \rel(J_j)$ for $1\leq i < j \leq k$. 
We claim that it is feasible to set $[\stime(J_i),\etime(J_i))$ to $[\max\{\rel(J_i), \etime(J_{i-1})\}, \stime(J_i)+\w(J_i))$ for all $ 1<i\leq k$ and $[\stime(J_1), \etime(J_1)) = [\rel(J_1), \rel(J_1)+\w(J_1))$. 

We observe that $\den(J_1)\leq 1$ since $\sum_i \den(J_i) \leq 1$. 
It is feasible to set $[\stime(J_1),\etime(J_1))$ to $[\rel(J_1), \rel(J_1)+\w(J_1))$ since the input is feasible. 
Then we have to prove that 
$[\stime(J_i), \etime(J_i)) = [\max\{\rel(J_i), \etime(J_{i-1})\}, \stime(J_i)+\w(J_i)) \subseteq [\rel(J_i), \dl(J_i))$. 
It is easy to see that $\stime(J_i)\geq \rel(J_i)$ %\pw{[PW: why do we want to prove that $\stime(J_i)\leq \rel(J_i)$??? To be feasible, we need to start no earlier than the release time, i.e., we need $\stime(J_i)\geq \rel(J_i)$]}. 
Furthermore, $\sum_{g\leq i}\den(J_g)\leq 1$. That is, $\sum_{g\leq i} \frac{\w(J_g)}{\dl(J_g)-\rel(J_g)} \leq 1$. 
From the ordering of jobs we have $1\geq \sum_{g\leq i}\frac{\w(J_g)}{\dl(J_g)-\rel(J_g)}\geq \sum_{g\leq i}\frac{\w(J_g)}{\dl(J_i)-\rel(J_1)}$. 
Hence~%\pw{[PW: Namely??? do you want to say ``therefore'' or ``hence'']}
, $\sum_{g\leq i}\w(J_g) \leq \dl(J_i)-\rel(J_1)$. 
Therefore $J_i$ can be finished before $\dl(J_i)$.
\end{proof}

\runtitle{Algorithm $\AlgAgree$.}
The algorithm consists of the following components: InsertQueue, SetStartTime and ScheduleQueue.

\noindent
\textbf{\emph{InsertQueue:}}
We keep a counter $q$ for the number of queues created.
When a job~$J$ arrives, if $\den(J) + \sum_{J' \in \queue_q} \den(J') \leq 1$,
then job $J$ is added to $\queue_q$;
otherwise, job $J$ is added to a new queue $\queue_{q+1}$ and we set $q \leftarrow q+1$.

\noindent
\textbf{\emph{SetStartTime:}}
For the current queue, we keep a current ending time $E$, initially set to $0$.
When a new job $J$ is added to the queue, if $\rel(J) \leq E$,
we set $\stime(J) \leftarrow E$;
otherwise, we set $\stime(J) \leftarrow \rel(J)$.
We then update $E$ to $\stime(J)+\w(J)$.

\noindent
\textbf{\emph{ScheduleQueue:}}
At any time~$t$, schedule all jobs in all queues with start time set at $t$.

By Lemma~\ref{thm:horizontal_density},
the schedule returns by $\AlgAgree$ is feasible.
We then analyze its load and hence derive its competitive ratio.
Recall the definition of $\IL{1}$ and $\IS{1}$

\begin{lemma}
\label{thm:agree_load}
Using $\AlgAgree$, we have
(i) $\load(t)\leq 3\cdot\lceil\avg(t)\rceil$ for $t\in\IL{1}$; 
(ii) $\load(t)\leq \hhl{1}$ for $t\in\IS{1}$.
\end{lemma}

\begin{proof}
% \pw{[PW: to be filled in by AL/HL.]}
%
For timeslot $t$, suppose there are $k$ queues ($Q_1, Q_2, \cdots, Q_k$) which contains jobs available at $t$. 
According to our algorithm, $\load(\AlgAgree,t)\leq k$.


Let $D_i$ be the sum of densities of jobs in $Q_i$
%~\pw{[PW: $Q_i$???]}
. Consider $t\in\IL{1}$. 
By the InsertQueue procedure
%~\pw{[PW: InsertQueue procedure???]}
, $D_i+D_{i+1}>1$ for $1<i<k-1$. 
Therefore, $\avg(t) = \sum_{1\leq i\leq k}D_i 
> \sum_{2\leq i \leq k-1} D_i 
\geq \lfloor\frac{k-2}{2}\rfloor 
= \lfloor\frac{k}{2}\rfloor-1$. 
It can be shown that $k\leq 3\cdot \lceil\avg(t)\rceil$ since $\avg(t)>1$.\footnote{%
Given $\lfloor\frac{k}{2}\rfloor-1<a$ where $a$ is a real number and $k$ is integral, we have $\frac{k}{2}-1<\lfloor\frac{k}{2}\rfloor<a+1\leq \lceil a\rceil+1$. Hence, $k< 2\lceil a\rceil+2$. 
Because both sides are integral, $k\leq 2\lceil a\rceil+1$. 
Furthermore, $k\leq 3\lceil a\rceil$ if $a>0$.} 
That is, $\load(t)\leq 3\lceil \avg(t)\rceil$ for $t\in\IL{1}$.

For $t\in\IS{1}$, $\avg(t)\leq 1$ by definition. That is, the sum of densities of all available jobs at $t$ is no more than $1$. 
By the InsertQueue procedure
%~\pw{[PW: InsertQueue procedure???]}
 all jobs will be in the same queue. Hence $\load(t)\leq 1$ for $t\in\IS{1}$.
\end{proof}

By Lemma~\ref{thm:agree_load} and Theorem~\ref{thm:horizontal_framework}, we have Theorem~\ref{thm:agree_cr} by setting $c=3$ and $c'=1$.
\begin{theorem}
\label{thm:agree_cr}
For jobs with unit height, arbitrary width and agreeable deadlines,
$\AlgAgree$ is $(\frac{(12\alpha)^\alpha}{2}+1)$-competitive.
\end{theorem}

\begin{corollary}
For jobs with unit height, arbitrary width and same release time or same deadline, 
the competitive ratio can be improved to $(\frac{(8\alpha)^\alpha}{2}+1)$ by using first-fit instead of next-fit for InsertQueue. 
\end{corollary}



